Adaptive continuity-preserving simplification of street networks

Street network data is widely used to study human-based activities and urban structure. Often, these data are geared towards transportation applications, which require highly granular, directed graphs that capture the complex relationships of potential traffic patterns. While this level of network detail is critical for certain fine-grained mobility models, it represents a hindrance for studies concerned with the morphology of the street network. For the latter case, street network simplification - the process of converting a highly granular input network into its most simple morphological form - is a necessary, but highly tedious preprocessing step, especially when conducted manually. In this manuscript, we develop and present a novel adaptive algorithm for simplifying street networks that is both fully automated and able to mimic results obtained through a manual simplification routine. The algorithm - available in the neatnet Python package - outperforms current state-of-the-art procedures when comparing those methods to manually, human-simplified data, while preserving network continuity.

==> figures/fig_algo-diagram.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/fig_algo-diagram.png}
    \caption{Conceptual diagram of the proposed simplification algorithm. Input street network (0) undergoes topological verification and adaptation (1) before face artifact detection (2). The face artifacts are then classified based on contiguity of polygons and continuity of edges forming them (3). The result goes through the geometry replacement pipeline that alters the existing geometry (4) based on the artifact classification to ensure minimal change and preservation of main network characteristics. Steps 2-4 are then repeated before returning the output consisting of a simplified street network.}
    \label{fig:algo-diagram}
\end{figure}

==> figures/fig_allmethods.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/fig_allmethods.png}
    \caption{Output of different simplification methods for a street network fragment in Seraing, Liège (Belgium).}
    \label{fig:allmethods}
\end{figure}

==> figures/fig_ces.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/fig_ces.png}
    \caption{A subset of the CES typology derived from the Liège street network. A single CES type is composed of the number of nodes forming the artifact and the continuity types of strokes forming its boundary. For example, the most common type, 3CES, is composed of 3 nodes and 3 continuity strokes, one of each kind, while 5S is composed of 5 nodes and a single continuity stroke of type S (as it never leaves the artifact). The total number of CES types is theoretically infinite given no upper bound on number of nodes exists. The full overview of types present in Liège is available in Appendix \ref{appendix:ces}.}
    \label{fig:ces}
\end{figure}

==> figures/fig_ces_liege_post_parts.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/ces_liege_post_part1.png}
    \caption{CES typology derived from Liège street network (part 1).}
    \label{fig:ces1}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/ces_liege_post_part2.png}
    \caption{CES typology derived from Liège street network (part 2).}
    \label{fig:ces2}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/ces_liege_post_part3.png}
    \caption{CES typology derived from Liège street network (part 3).}
    \label{fig:ces3}
\end{figure}

==> figures/fig_chi-buildings.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/fig_chi-buildings.png}
    \caption{Chatterjee's $\xi$ correlation coefficient between properties of networks that are~(a)~manually simplified (``manual''),~(b)~simplified by our proposed method (``neatnet''),~(c)~simplified by our proposed method after applying a building exclusion mask (``neatnet-buildings''),~vs.~the original network as a baseline. Higher is considered better -- approaching $1.0$ on the $y$-axis. For all seven considered metrics and in all seven considered cities, adding the building exclusion mask slightly increases the $\xi$ correlation coefficient, bringing it closer to a value of $1.0$.
    }
    \label{fig:chi-buildings}
\end{figure}

==> figures/fig_chi.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/fig_chi.png}
    \caption{Chatterjee's $\xi$ correlation coefficient between properties of manually simplified networks and networks based on each of the tested algorithms vs.~the original network as a baseline. Higher is considered better -- approaching $1.0$ on the $y$-axis.}
    \label{fig:chi}
\end{figure}

==> figures/fig_delta-buildings.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/fig_delta-buildings.png}
    \caption{Euclidean distance between properties of networks that are~(a)~manually simplified (``manual''),~(b)~simplified by our proposed method (``neatnet''),~(c)~simplified by our proposed method after applying a building exclusion mask (``neatnet-buildings''), vs.~the original network as a baseline. Lower is considered better -- approaching $0.0$ on the $y$-axis. For all seven considered metrics and in all seven considered cities, adding the building exclusion mask slightly decreases the Euclidean distance between the distributions, bringing it closer to a value of $0.0$.
    }
    \label{fig:delta-buildings}
\end{figure}


==> figures/fig_delta.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/fig_delta.png}
    \caption{Euclidean distance between properties of manually simplified networks and networks based on each of the tested algorithms vs.~the original network as a baseline. Lower is considered better -- approaching $0.0$ on the $y$-axis.}
    \label{fig:delta}
\end{figure}

==> figures/fig_original-manual.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/fig_original-manual.png}
    \caption{Illustration of the simplification process by the example of a street network fragment in Seraing, Liège (Belgium).~(a)~The left panel shows the input data, downloaded from OpenStreetMap \citep{openstreetmap_contributors_openstreetmap_2025}, before simplification. Due to transportation-focused mapping, the input network contains several intersections, roundabouts, and dual carriageways that are mapped with a high level of granularity.~(b)~The same network after simplification. The level of granularity has been reduced where appropriate, so that every intersection is represented by one node and every street segment is represented by one edge.}
    \label{fig:original-manual}
\end{figure}

==> figures/fig_situations-selection.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/fig_situations-selection.png}
    \caption{A small set of example situations that ought to be simplified and the resutling simplified networks from all tested methods, together with the comparison to the manual simplification considered ground truth.}
    \label{fig:situations-selection}
\end{figure}
